AntShield: On-Device Detection of Personal Information Exposure

Mobile devices have access to personal, potentially sensitive data, and there is a growing number of applications that transmit this personally identifiable information (PII) over the network. In this paper, we present the AntShield system that performs on-device packet-level monitoring and detects the transmission of such sensitive information accurately and in real-time. A key insight is to distinguish PII that is predefined and is easily available on the device from PII that is unknown a priori but can be automatically detected by classifiers. Our system not only combines, for the first time, the advantages of on-device monitoring with the power of learning unknown PII, but also outperforms either of the two approaches alone. We demonstrate the real-time performance of our prototype as well as the classification performance using a dataset that we collect and analyze from scratch (including new findings in terms of leaks and patterns). AntShield is a first step towards enabling distributed learning of private information exposure.

==> 02-motivation.tex <==
\section{Motivation} \label{sec:problem}


\subsection{Problem Definition and Scope \label{sec:problem-leak}} %

{\bf Defining PII.} Mobile devices have access to wealth of resources and information, much of which is personal and potentially sensitive. We will refer to such  personally identifiable information as {\em PII} and examples include:
%
\begin{itemize}
%
\item Device Identifiers: IMEI, AndroidID, phone number, serial number, ICCID, MAC Address.
%
\item User identifiers: credentials (per app, usually transmitted over HTTPS), advertiserID, email.
%
\item User demographic: (1) first/last name, gender, zipcode, city, \etc - unavailable through Android APIs, and (2) location - available through Android API
%
\item User-defined: the user can also define any custom string that should be monitored  (\eg see GUI in Fig. \ref{fig:guiPI}), such as digits of her credit card.
%
%
\end{itemize} 


The list is consistent with prior work \eg \cite{recon15}, but 
 clearly not exhaustive. For example, it does not include photos, videos, and other data collected through various sensors on the mobile. 
%
The above PII can be further classified across different dimensions. Some of them are static (\ie hard coded on the phone and never change), while other are dynamic (such as location or email accounts). Some of them can be pulled by any application via API calls (IMEI, MAC address, phone number, \etc), and some are hidden from apps, unless the apps explicitly ask the user for this information (name, gender, password, \etc).
%
A key insight of this paper is the distinction between \preDefLeak PII (available via Android APIs) and PII that is hidden from apps and referred to as \unknownLeak PII throughout the paper. The main distinction is whether the PII string is known apriori on the device or not.  Our system employs different techniques for \preDefLeak PII (\stringMatch) and \unknownLeak PII (machine learning).

{\bf Exposure of PII.} Many mobile apps access, process and transmit some of this information over the network. Sometimes this is necessary for the app to operate (\eg it is not a surprise that GoogleMaps will need the location, or that the Facebook app will transmit user credentials to a FB server). However this is not always the case: apps (or third party libraries used by apps) may transmit sensitive information to adservers, trackers or malicious servers, without the user being aware. Although the user has control over the permissions granted to apps at installation time, permissions are not sufficient since (i) users typically accept by default to install apps; (ii) permissions do not protect against inter-app  communication and  poorly documented system calls; and (iii) they do not capture run-time behavior. We refer to the transmission of a packet from the device to the network,  containing at least one  PII, as a {\em privacy exposure}. 

%
We avoid the term  {\em privacy leak}, because  whether the transmission of the PII is an actual leak depends on the intent of the transmission: \ie, whether it is necessary for the operation of the app, malicious or honest-but-curious attacker, acceptable or not to the user. Users may be even willing to accept the sharing of their personal data in exchange for some service  or monetary benefit; however, users today are typically unaware of which personal data are actually exposed over the network and  for what purpose. Distinguishing between privacy exposure and an actual privacy leak is out of the scope of this paper.\footnote{Throughout the paper, we may use at place the terms ``exposure'' and ``leak'' interchangeably to mean ``exposure'', as defined above.}   

{\bf Goal.} Our goal, in this paper, is to {\em detect the transmission of PII over the network} and make the user aware of that. We consider the transmission of packets with PII over clear text or SSL, to an app's server or a third party server. Our goal is to design a system that identifies all this PII exposed over the network, and raise the user's awareness.  (The user may decide to allow the transmission, block it, or obfuscate it.) In this paper, we explore to what extent PII can be detected in a {\em distributed way}, on the device, accurately and with low overhead.  

\subsection{Design Rationale \label{sec:problem-mobile}}


Below we describe our objectives and how they guide our design choices to achieve our goal.

%
{\bf VPN-based.} First, we want a solution that is accessible to  the non-sophisticated end-user.  This rules out solutions that require rooting the phone - the solution has to be a mobile app that the user can simply install, enable in the background, and occasionally interact with (\eg notification about suspicious activity, or by occasionally checking PII reports).  At the same time, we need to be able to intercept and inspect every packet in and out of the device, which is not possible from user space, in any other way today, other than using the VPN service available both in Android and iOS.

{\bf On-device.} Second, we want to provide a solution that operates purely on the device and does not redirect traffic through a middle server. This has several advantages: it does not need to expand the trust base (data does not need to leave the user's device), and it is well positioned to have access to rich information available on the device  (app names, and predefined PII). It also poses implementation challenges, as it requires to translate every connection from layer-3 to layer-4 and vice versa, and this is non-trivial to implement efficiently \cite{antmonitor-arxiv}. To that end, we build on prior work by \anteater, which is the most efficient implementation (in terms of throughput, battery and other resources)  to the best of our knowledge today.\footnote{\anteater is currently available only on the Android platform, but it can be ported to run on iOS as well, since all it requires is the VPN service.}

{\bf Detecting PII. }Third, we want to be able to accurately detect a range of PII, both \preDefLeak (through fast DPI and string matching), and \unknownLeak through learning. Towards the first goal, we utilize the DPI module provided by \anteater; see Sec. \ref{sec:system-sdk} and \cite{antmonitor-arxiv}. Towards the second goal, we build on and improve the classifiers produced by \recon, previously done only in a centralized way; see Sec. \ref{sec:recon} and \cite{recon15}. 

{\bf Put user in control.} Users can decide how much PII to give to the system:  the more PII is provided to \antshield, the better the detection accuracy.
%
Users also have full control of if/how much ground truth to share for training with other users to enjoy the benefits of crowdsourcing. They can pick whether to label \preDefLeak leaks only, or they can manually add more \unknownLeak strings to search for. Moreover, users can also choose which applications' packets to contribute. For instance, they can decide to contribute data for gaming apps only, but not for sensitive apps, such as Chrome and Gmail. %

==> 04-1-application-privacy.tex <==

\subsection{Application I: Privacy Leaks}
\label{sec:leakage}


Mobile devices today have access to personally identifiable information (PII) and they routinely leak it through the network, often to third parties without the user's knowledge.  PII includes:  (i) mobile phone IDs, such as IMEI (which uniquely identifies a device within a mobile network), and Android Device ID; and (ii) information that can uniquely identify the user (such as phone number, email address, or even credit card) or other information (e.g. location, demographics). 
%
 Sometimes sending out PII is necessary for the operation of the phone (\eg  a device must identify itself to connect to a wireless network) or of the apps (\eg location must be obtained for location-based services). However, the leak may not serve the user (\eg going to advertisers or analytics companies) or may even be malicious. Leaks in plain text can be intercepted by listening third parties, \eg in public WiFi networks.
Although modern mobile platforms (Android, iOS, Windows) require that apps obtain permission before requesting access to certain resources, and  isolate apps (execution, memory, storage) from each other, this is not sufficient to prevent information from leaking out of the device, \eg due to interaction between apps \cite{felt2011permission}.  Even worse, users are unaware of how their data are used \cite{lin2012expectation}. 
%




\begin{table}
	\centering
	{\scriptsize
		\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|}
			\hline
			{\bf App Name} &  {\bf Leak Type}  & {\bf \# Flows}\\
			\hline
			  VnExpress.net  & \multirow{2}{*}{ \parbox{2.2cm}{IMEI, Phone\#, Location, Email, DeviceID} }  & 33147 \\
				  &  & \\
			  Zing Mp3  & \xspace IMEI, DeviceID  & 14745 \\
			  Clean Master & \xspace DeviceID  & 1768 \\
			  WiFi Maps  & \xspace IMEI, Location  & 1582 \\
			  Relay for reddit  & \xspace Location  & 638 \\
			  System  &  \multirow{2}{*}{  \parbox{2.2cm}{IMEI, Location, DeviceID} }  & 301 \\
                                   &  & \\
			  Chrome  & \xspace Location  & 143 \\
%
			  ES File Expl.  & \xspace DeviceID  & 96 \\
			  MyFitnessPal  & \xspace Location  & 76 \\
			  DR Radio  & \xspace DeviceID  & 68 \\
			  Speedtest & \xspace Location  & 48 \\
			  DexKnows  & \xspace IMEI,Location  & 47 \\
			  Skype   & \xspace IMEI, DeviceID  & 42 \\
%
			  iWindsurf  & \xspace IMEI, Location  & 22 \\			  		
 			  WhatsApp &  Phone\#  & 20 \\	  			  			  
%
%
%
%


			$\cdots$ & $\cdots$ & $\cdots$ \\
			\hline
			  All & All & 52923 \\
			\hline
		\end{tabular}
		\quad
		\begin{tabular}{|@{}l@{}|l@{}|}
			\hline
			{\bf Domain Name} &   {\bf \# Flows}\\
			\hline
			eclick.vn. & 8760 \\
			api.mp3.zing.vn. & 7561 \\
			ksmobile.com. & 620 \\
			zaloapp.com. & 332 \\
			ngoisao.net. & 209 \\
			api.staircase3.com. & 150 \\
			openweathermap.org. & 47 \\
			adtima.vn. & 36 \\
			ads.adap.tv. & 31 \\
			apps.ad-x.co.uk. & 30 \\
			adkmob.com. & 27 \\
			whatsapp.net. & 27 \\
			mopub.com. & 25 \\
			duapps.com. & 25 \\
			api.dexknows.com. & 24 \\
%
			server.radio-fm.us. & 15 \\
			inmobi.com. & 14 \\
%
%
			$\cdots$ & $\cdots$ \\
			\hline
			All & 18020 \\
			\hline
		\end{tabular}
	}
	%
	\caption{{\small Flows Leaking PII found in the collected data. (Note: the number of flows at the left (52923) is higher than at the right (18020) because we count a flow that leaks multiple PIIs multiple times.)}}
	%
	\label{tab:leaks}
\end{table}


{\bf Privacy Leaks Detection and Prevention Module.} \label{sec:privacy-design}
%
%
We extended the basic \anteater functionality with an analysis module that performs real-time DPI.  The user can define strings that correspond to private information that should be prevented from leaking; see screenshot in Fig. \ref{fig:guiPI}. Before sending out a packet, the \client inspects it and searches for any of those strings. By default, if the string is found, \anteater hashes it (with a random string of the same length, so as not to alter the payload length) before sending the packet out, and asks the user what to do in the future for the given string/app combination, as shown in Fig. \ref{fig:guiNotif}. The user can choose to allow future packets to be sent out unaltered, block them, or keep hashing the sensitive string (so that the application has a good chance to continue working but without the string being leaked). The system remembers the action to take in the  future for the same app and ``leak,'' and it will no longer bother the user with notifications. The user may also look at the history of the leaks, shown in Fig. \ref{fig:guiHistory}. \anteater can provides both {\em real-time} detection and {\em prevention}, on the mobile-device (not at the server) thanks to its efficient implementation, while \haystack and \pguard do not achieve both; and \recon can achieve the same on the server, and could gracefully run on top of \anteater as well. Specifically, \anteater can inspect a packet for leaks in <10 ms (Sec. \ref{sec:Other Metrics}), and it was the first app to demonstrate this real-time capability in \cite{antmonitor-poster-mobicom15}.
%

{\bf Encrypted Traffic. } Since we require plain text in order to perform DPI, and much of the traffic is encrypted, we developed a TLS proxy that uses the SandroProxy library \cite{sandro-proxy}, also used by \pguard,  to intercept secure connections, decrypt the packets, and then re-encrypt them before sending them to their intended Internet hosts. This method works for most apps, but it cannot intercept traffic from highly sensitive apps, such as banking apps, that use certificate pinning. Due to the intrusive nature of intercepting TLS/SSL traffic, we allow users to disable this option.


\begin{figure}[t!]
%
\centering
\includegraphics[width=0.45\textwidth]{figs/adservers_nbytes_v2.pdf}
%
%
\caption{Amount of traffic sent to ad \& analytics servers} 
%
\label{fig:adservers}
\end{figure}


{\bf Privacy Leaks Detected.} %
We analyzed the data collected from our user study, and found a large number of privacy leaks in plain text. Table \ref{tab:leaks} presents the apps and destination domains with the highest number of flows leaking. The worst offender in the list was the app \textvtt{VnExpress.net} that leaked five different types of PII up to 33,145 times towards the domain \textvtt{eclick.vn} -- an advertising network. The list of leaking apps includes very popular apps with tens of millions of downloads, such as Skype and WhatsApp, and the list of domains includes many  mobile ad networks (such as \textvtt{mopub, inmobi, adkmob, adtima}). 
%
Using the data collected by \anteater at the users' mobile devices, we calculated the amount of data that is transmitted from/to  ad networks, analytics and mediation services. %
 Fig. \ref{fig:adservers} shows that the amount of traffic transmitted towards such servers for the top 20 domains is in the order of GBs, consists of several domains, and tens of thousands of flows per domain. Fig. \ref{fig:guiVisual} visualizes the destinations for one device: it shows which apps leak information to which destinations. %

%

{\bf Discussion.} The inherent advantage of \anteater in this domain is that it runs on the device, which is a more attractive place for users to perform PII scrubbing than a middlebox, since sensitive data does not have to leave the device. Traffic encrypted at the application level can also be intercepted and inspected by the TLS proxy in \anteater, then re-encrypted, if the user chooses to do so (by agreeing to install a root certificate). One limitation of our current approach is that PII leakage is detected using string matching, which can be evaded by a more sophisticated  attacker, who can leak information across multiple packets or by encoding the text to be leaked. At its current state, our privacy  leaks detection is mostly useful for raising awareness of the magnitude, nature and cost of PII leaking, and can be useful in the case of an honest-but-curious adversary. For example, a legitimate app that leaks information to trackers is likely to stop doing so if users become aware and start uninstalling the app. The on-device visualization shown on Fig. \ref{fig:guiVisual} displays the destination (IP address, hostname/domain, and type of server) to which each app sends data for all active connections and it is updated in real-time. Another inherent advantage of running privacy leak detection on the device (as opposed to the middle server) is the access to contextual information available on the device (such as the app that generated the traffic), which can be used to detect more sophisticated PII leaks with machine learning.
